LPV Modeling of the Atmospheric Flight Dynamics of a Generic Parafoil Return Vehicle

Obtaining models that can be used for control is of utmost importance to ensure the guidance and navigation of spacecraft, like a Generic Parafoil Return Vehicle (GPRV). In this paper, we convert a nonlinear model of the atmospheric flight dynamics of an GPRV to a Linear Parameter-Varying (LPV) description, such that the LPV model is suitable for navigation control design. Automated conversion methods for nonlinear models can result in complex LPV representation, which are not suitable for controller synthesis. We apply several state-of-the-art techniques, including learning based approaches, to optimize the complexity and conservatism of the LPV embedding for an GPRV. The results show that we can obtain an LPV embedding that approximates the complex nonlinear dynamics sufficiently well, where the balance between complexity, conservatism and model performance is optimal.

==> Sections/Introduction.tex <==
\section{Introduction}
\begin{itemize}
	\item What is the Space Rider
	\item The control problem and why an LPV controller
	\item Need for an LPV model and a small scheduling vector dimension
	\item Introduction to scheduling dimension reduction 
\end{itemize}
The European Space Agency (ESA) is currently developing the Space Rider (SR), to perform research in low orbit. The SR is a re-usable module. Hence, it is designed to return to the surface of the earth and make a precision landing at a predefined location, i.e. landing with a bounded location and a bounded velocity. The last stage of the re-entry procedure of the SR is the terminal descent phase. During this phase the SR is navigated to its landing point by means of a guided parafoil. This is shown in Figure \ref{fig:Intro:SR}. The navigation is challenging, since the dynamics of the SR with the parafoil are highly coupled and nonlinear \cite{DeLange2021}. Moreover, wind disturbance is acting on the system.\\
\begin{figure}
	\begin{center}
		\includegraphics[width=8.4cm]{Figures/Space_Rider_2.eps}    % The printed column width is 8.4 cm.
		\caption{The Space Rider with the parafoil} 
		\label{fig:Intro:SR}
	\end{center}
\end{figure}\\
One of the considered control strategies for the Space Rider is Linear Parameter Varying (LPV) control via $\mathcal{L}_2$-gain controller synthesis. This approach requires the nonlinear model to be transformed into an LPV model with a scheduling vector. To keep the synthesis problem feasible it is important that the dimension of the scheduling vector is below 5 \hl{cite?}. The complexity of the control problem increases exponentially with the dimension of the scheduling vector. As does the conservatism in the convex scheduling hull if the dimension of the scheduling vector increases. In general the control problem becomes infeasible after a dimension of 5\hl{prove}.\\
\\
Multiple methods exists for scheduling dimension reduction. The two methods explored in this paper are principle component analyses (PCA) and a deep neural network (DNN) scheduling reduction. With PCA, the model variations are transformed with a set of orthogonal transformations to obtain a vector of linearly uncorrelated variations in contributing order. These transformations are obtained based on a data-set of the model variations. The dimension of the scheduling variable is reduced by disregarding the linearly uncorrelated variations with the lowest contributions. This will however impact the accuracy of the model. The DNN scheduling reduction trains a deep neural network to describe the relation from the states and input of the model to a reduced scheduling vector. A linear layer is trained from the reduced scheduling vector to the model variations. The DNN possible benefits from the freedom of finding any arbitrary mapping from the states and the input to the reduced scheduling variable. The PCA method uses a fixed nonlinear map from the state and input to the model variations and is limited to finding an affine linear map from these model variation to a reduced scheduling vector.\\
\\
This paper is structured as following. First the preliminaries on LPV modeling, normalization, the PCA method and the DNN method are given. Than the Space Rider model is introduced and the and the discussed methods are applied to obtain an LPV model and a reduced scheduling reduction. The results will show the accuracy of the model variations versus the scheduling dimension. The accuracy of the model is related to the obtained derivative from the model. Lastly a conclusion is given over the used methods based on the obtained results.

==> Sections/Problem_Statement.tex <==
\section{Problem Statement!}
The fight dynamics of the SR guided by a parafoil is a highly nonlinear and coupled system. The design of the control solution needs to navigate and land the SR at a predefined location. This is challenging due to wind disturbances. One approach to guarantee the performance of control solution is by applying LPV control and $L_2$-gain synthesis. This gives the need for an LPV model, with a low scheduling dimension. controller synthesis with a scheduling dimension higher as five is not tractable. By systematically scheduling all varying matrix functions in the model a baseline LPV model for the SR with parafoil is created, but this gives 71 scheduling variables. This paper will show how to reduce the scheduling dimension, how the reduction impact the accuracy of the model and how to model performance is quantified.
